Flash-LLM: Enabling Cost-Effective and Highly-Efficient Large Generative Model Inference with Unstructured Sparsity

With the fast growth of parameter size, it becomes increasingly challenging to deploy large generative models as they typically require large GPU memory consumption and massive computation. Unstructured model pruning has been a common approach to reduce both GPU memory footprint and the overall computation while retaining good model accuracy. However, the existing solutions do not provide a highly-efficient support for handling unstructured sparsity on modern GPUs, especially on the highly-structured Tensor Core hardware. Therefore, we propose Flash-LLM for enabling low-cost and highly-efficient large generative model inference with the sophisticated support of unstructured sparsity on high-performance but highly restrictive Tensor Cores. Based on our key observation that the main bottleneck of generative model inference is the several skinny matrix multiplications for which Tensor Cores would be significantly under-utilized due to low computational intensity, we propose a general Load-as-Sparse and Compute-as-Dense methodology for unstructured sparse matrix multiplication. The basic insight is to address the significant memory bandwidth bottleneck while tolerating redundant computations that are not critical for end-to-end performance on Tensor Cores. Based on this, we design an effective software framework for Tensor Core based unstructured SpMM, leveraging on-chip resources for efficient sparse data extraction and computation/memory-access overlapping. At SpMM kernel level, Flash-LLM significantly outperforms the state-of-the-art library, i.e., Sputnik and SparTA by an average of 2.9x and 1.5x, respectively. At end-to-end framework level on OPT-30B/66B/175B models, for tokens per GPU-second, Flash-LLM achieves up to 3.8x and 3.6x improvement over DeepSpeed and FasterTransformer, respectively, with significantly lower inference cost.

==> Chapters/6-Discussion.tex <==
\section{Discussion}

This paper mainly addresses the memory footprint problem of large generative models by supporting pruned models on tensor cores efficiently.
% As discussed in Sec.\ref{sec:motivation}, this paper aims to support unstructured sparsity for better accuracy.
\SYS{} can efficiently support the SpMM for generative models with a sparse ratio of 70\%-90\%.
In practice, retaining high accuracy on this range of sparse ratios requires retraining-based pruning~\cite{liu2018rethinking, han2015learning} rather than the post-training pruning~\cite{SparseGPT}.
The retraining-based pruning consumes a high fine-tuning cost,
which as a result becomes one limitation of \SYS{}.
Quantization is another common compression approach to reduce memory footprint, which is orthogonal to pruning and can be combined with pruning together.

\TODO{Remove this section if there is no space. Most content of this section is already in the related work section.}
